UKP-SQUARE: An Online Platform for Question Answering Research

Recent advances in NLP and information retrieval have given rise to a diverse set of question answering tasks that are of different formats (e.g., extractive, abstractive), require different model architectures (e.g., generative, discriminative), and setups (e.g., with or without retrieval). Despite having a large number of powerful, specialized QA pipelines (which we refer to as Skills) that consider a single domain, model or setup, there exists no framework where users can easily explore and compare such pipelines and can extend them according to their needs. To address this issue, we present UKP-SQUARE, an extensible online QA platform for researchers which allows users to query and analyze a large collection of modern Skills via a user-friendly web interface and integrated behavioural tests. In addition, QA researchers can develop, manage, and share their custom Skills using our microservices that support a wide range of models (Transformers, Adapters, ONNX), datastores and retrieval techniques (e.g., sparse and dense). UKP-SQUARE is available on https://square.ukp-lab.de.

==> sections/evaluation.tex <==
For the successful adoption of our platform in a practical setting, aspects of accuracy, speed and hardware constraints should be taken into account. Therefore, in this section, we evaluate the performance of the models deployed on our platform in terms of their accuracy, speed, and memory usage.

\begin{table*}
\centering
\scalebox{1}{
\begin{tabular}{@{}llll@{}}
\toprule
Model & Accuracy & Inference time (ms) & Memory usage \\ \midrule
dpr & \% &  1 & - \\
 \\ \bottomrule
\end{tabular}
}
\caption{Performance benchmarks of models deployed to the UKP SQuARE v1.0 platform. } \label{tab:model_benchmarking}


\end{table*}

==> sections/related_work.tex <==
Recent research in QA systems has primarily focused on open-domain QA \cite{karpukhin2020dense, lee2021learning} using dense retrieval techniques. While these systems perform reasonably well for a diverse set of questions, they do not work well with domain specific user queries where precise knowledge on the subject is required. Moreover, these systems predominantly use the wikipedia dumps for information retrieval. In comparsion, our QA system caters to a wide variety of QA domains through SOTA neural models (HF, adapters, ONNX) and datasets (NQ, MS MARCO, BioASQ). \cite{levy2021opendomain} introduce an open-domain QA system for emergent domains such as COVID-19 but it is largely restricted to the medical domain. \\
The previously discussed QA systems use dense retrieval techniques which may not be the best choice in practical real-time QA systems since it introduces additional complexity, memory and time inefficiency and are not interpretable. To tackle this issue, the authors in \cite{dibia2020neuralqa} introduce NeuralQA, an interactive tool for QA that leverages the benefits of sparse retrieval along with the reader models from the HF API. Additionally, their system supports visualization of gradient-based explanations to support qualitative inspection of model behaviour.  The only downside of using such a system is the inability of the retriever to retrieve semantically similar documents since sparse retrieval relies on exact matching. With our system, we leverage the benefits of both sparse and dense retrieval systems by providing an option to use any one of them based on the end-user's choice and feasibility.  \\
In recent years, a huge emphasis has been laid on the interpretability of QA systems. One such system called \mbox{MODULARQA} has been developed by Khot et al. in their work \cite{khot2021text}. \mbox{MODULARQA} can answer and explain complex multi-hop reasoning questions by decomposing them into simpler sub-questions answerable by a neural factoid single-span QA model and a symbolic calculator. Though this system provides easy-to-interpret explanations of its reasoning, it can only work for DROP \cite{Dua2019DROP} and HotpotQA \cite{yang2018hotpotqa} datasets which limits its use in practical QA systems. With our system, we support a plethora of models trained on datasets encompassing all the different QA domains.\\
To the best of our knowledge, there are no existing QA systems that cover a multitude of models for different QA components (retrievers, rerankers, readers/generators) and flexible index datastores (Elastic search, FAISS) which allow the users to adapt them for their particular tasks. The closest framework that relates to our work is Haystack\footnote{\url{https://haystack.deepset.ai/overview/intro}}. Haystack is an open-source framework for building search systems that work intelligently over large document collections. It supports all the latest models from the HF API, different index datastores such as Elastic search, FAISS, Milvus, and SQL, and can be scaled to large applications. The major difference between our QA system and Haystack is that the latter has to be set up by the users on their own infrastructure and the user has to familiarize with the framework in order to use it. Moreover, our QA system features model explainability using CheckList \cite{ribeiro2020accuracy} and provides a wider choice of models including adapters \cite{pmlr-v97-houlsby19a} from the adapterhub \cite{pfeiffer2020adapterhub}.

